Guillotine and Tiling Cofiniteness in Unary Picture Languages

Motivated by the study of closure operations on picture languages, we ask when a set of unary tiles can generate all sufficiently large pictures either via repeated horizontal and vertical concatenations or via tiling operations. In one dimension, the lengths of words in the concatenation closure of a unary language form an additive subsemigroup of positive natural numbers; hence, they are finitely generated. Cofiniteness is characterized by the gcd of these generators being one. Since ordinary cofiniteness in two dimensions is too restrictive and essentially reduces to degenerate one-dimensional conditions on strips, we introduce and study asymptotic cofiniteness: all sufficiently large rectangular pictures are generated. A direct extension of the one-dimensional criterion, requiring the gcd of the tile heights and of the tile widths to be one, is not sufficient, because local congruence obstructions may persist in two dimensions. We give an exact arithmetic characterization of asymptotic cofiniteness for arbitrary, possibly infinite, sets of unary rectangular tiles. The characterization is the same for the guillotine closure, obtained by horizontal and vertical concatenation, and for the full tiling closure. For finite tile sets, the proof combines semigroup arguments and an explicit least-common-multiple stacking construction for sufficiency, while necessity is obtained by a roots-of-unity argument applying also to nonsliceable tilings. The extension to infinite tile sets follows from the finite-basis theorem for Klarner systems.

==> eptcsdata.tex <==
\providecommand{\firstpage}{275}
\providecommand{\publicationstatus}{M. Hospod\'ar et al. (Eds.): 17th International Conference \\on Automata and Formal Languages (AFL 2026)\\
EPTCS 451, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.451.19}{10.4204/EPTCS.451.19}}
\pdfoutput=1

